Blurred LiDAR for Sharper 3D: Robust Handheld 3D Scanning with Diffuse LiDAR and RGB

3D surface reconstruction is essential across applications of virtual reality, robotics, and mobile scanning. However, RGB-based reconstruction often fails in low-texture, low-light, and low-albedo scenes. Handheld LiDARs, now common on mobile devices, aim to address these challenges by capturing depth information from time-of-flight measurements of a coarse grid of projected dots. Yet, these sparse LiDARs struggle with scene coverage on limited input views, leaving large gaps in depth information. In this work, we propose using an alternative class of "blurred" LiDAR that emits a diffuse flash, greatly improving scene coverage but introducing spatial ambiguity from mixed time-of-flight measurements across a wide field of view. To handle these ambiguities, we propose leveraging the complementary strengths of diffuse LiDAR with RGB. We introduce a Gaussian surfel-based rendering framework with a scene-adaptive loss function that dynamically balances RGB and diffuse LiDAR signals. We demonstrate that, surprisingly, diffuse LiDAR can outperform traditional sparse LiDAR, enabling robust 3D scanning with accurate color and geometry estimation in challenging environments.

==> sec/old/3_insight_old.tex <==
\section{Tradeoffs between SPADs and RGB for Mixed-texture Reconstruction}
\label{sec:insight}


\subsection{Setup and Problem Definition}

\sectionbf{Experimental Setup}
We propose integrating low-cost single-photon avalanche diode (SPAD) cameras with RGB sensors for efficient 3D surface reconstruction in mixed-texture scenes. Specifically, we model a setup with an 8x8 resolution SPAD camera with a fixed field-of-view, where a diffuse laser co-located with the SPAD emits a flood light pulse; this is unlike traditional experimental setups that use a collimated laser and focused detector. The SPAD records the time-of-flight ($t$) of returning photons, organizing the signals into transient histograms. Let $h(u, v, k)$ represent the histogram at pixel $(u, v)$, where $k$ indexes time bins; histogram bin widths reflect the SPAD's timing resolution, which determines the resolvable depth accuracy. By analyzing the distribution of photon counts over $N_t$ bins, referred to as "transients," depth distribution over each pixel's field-of-view can be inferred, with finer temporal resolution yielding more precise estimates.

We further model a capture setup with co-located SPAD and RGB cameras, performing multiple captures of a scene. The sensors are jointly calibrated, and the camera pose is assumed to be known; in real settings, ground truth poses are estimated using COLMAP from the RGB inputs. We propose that the combination of low-cost SPADs, producing transient histograms, and RGB data, producing dense texture information, enables detailed 3D reconstruction of mixed-texture scenes in a compact, low-cost system. 

\sectionbf{Transients from Low-Cost SPADs} Each pixel $(u, v)$ of the 8x8 SPAD array captures photon arrival times from a diffuse light pulse. The transient response for a pixel $(u, v)$ can be expressed as:

\[
\tau_{(u, v)}(t) = \int_S \rho(x) \frac{G(x, \omega)}{||x||^4} \delta\left(\left\|x\right\| - \frac{ct}{2}\right) dA(x)
\]

where $\rho(x)$ is the surface albedo, $G(x, \omega) = f_r(x, \mathbf{n}_x, \omega) V(x, \omega)$ represents the Lambertian reflectance, visibility, and the bidirectional reflectance distribution function (BRDF), and $\delta$ is the Dirac delta function modeling the time delay based on distance. We ignore contributions from higher-order bounces due to their weak contribution under our scene conditions. \sid{should be $r^2$ for one bounce. Lot of times not even $r^2$ because you assume that your lens can focus reasonably well enough. Also, equation notation is confusing (e.g. what is A(x)?} 

\subsection{Low-Cost SPAD and RGB Tradeoffs}


The integration of low-cost SPADs and RGB sensors offers complementary strengths for 3D surface reconstruction, particularly in mixed-texture scenes. We summarize these tradeoffs in Table \ref{table:tradeoffs}. Low-cost SPADs provide metric depth via transient histograms, albiet with very low spatial resolution (in our case, 8x8 pixels). Further, unlike traditional LiDAR systems, low-cost SPADs may use flood illumination, capturing depth information across a wider scene field of view in each pixel, rather than at a single point. \sid{$\leftarrow$ this doesn't seem SPAD specific. I think it is more so leveraging the use of active illumination, combined with the SPAD sensitivity.} Despite their limited resolution, however, SPADs excel in textureless \sid{again, it's lidar that can handle single-view depth, not SPAD specifically. Also, LiDARs would also fail in multi-view case if you don't have good geometric features to latch onto.} and low-light regions where RGB sensors fail to capture reliable multi-view depth cues (see Figure \ref{fig:tradeoff_example}).

RGB sensors, on the other hand, deliver dense relative depth with sharp boundary details in well-lit, high-texture scenes. However, they depend heavily on lighting and texture, often yielding poor results in low-light or textureless areas. Concavities on textureless objects further exacerbate depth ambiguity, leading to inaccurate reconstructions (see Figure \ref{fig:tradeoff_example}). While earlier LiDAR+RGB approaches have achieved high-fidelity reconstructions from dense LiDAR depth, the key challenge is how to leverage the complementary advantages of low-cost SPADs and RGB sensors effectively.


\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/Strengths.png} % Adjust the width as needed
\caption{Tradeoffs between RGB and SPAD sensors in 3D reconstruction alongside strengths of the methods. \sid{This seems like it belongs in the related works section, not in the methods.}}
\label{fig:strengths_figure}
\end{figure}


\subsection{Time-Resolved Imaging}
Time-resolved imaging, such as LiDAR, operates by emitting short pulses of light and measuring the return times of incident photons, referred to as the \textit{time of flight} (ToF). Single-photon avalanche diodes (SPADs) are a common sensor type capable of measuring these so called \textit{transient} images (i.e. photons incident over time). 
Although the applications of SPADs are promising, they often rely on high-cost or laboratory-grade setups. In contrast, the focus of our work is to highlight the potential of low-cost SPADs to improve 3D scanning.

\noindent
\textbf{Traditional Methods.} SPADs are often used to exploit transient light transport, such as in fluorescence lifetime measurements \cite{lee2023caspi}, non-line-of-sight (NLOS) imaging \cite{raskar2020seeing,kirmani2009looking}, and seeing through scattering media \cite{faccio2020non,xin2019theory,velten2012recovering}. Traditional ToF methods often use transient images for scene reconstruction in controlled environments \cite{jayasuriya2015depth}, but these works typically assume spot illumination, where reconstruction is guided only by a sparse set of depth points. In contrast, we focus on using \textit{diffuse} LiDAR, meaning the scene is diffusely illuminated, presenting a distinct set of challenges.

\noindent
\textbf{Learned Methods.} In recent years, machine learning techniques, such as NeRF, have been applied to SPAD measurements across many 3D vision tasks, including depth estimation \cite{jungerman20223d}, 3D reconstruction \cite{klinghoffer2024platonerf, attal2021torf, malik2024transient}, material classification \cite{callenberg2021low}, and NLOS imaging \cite{shen2021non, mu2022physics, fujimura2023nlos}. We focus on surface reconstruction from low-cost diffuse SPAD sensors. Recent work has explored using transient images from low-cost SPAD sensors to infer planar \cite{sifferman2023unlocking} and 3D surfaces \cite{mu2024towards}. Yet, while these works highlight the feasibility of low-cost SPADs for 3D vision, they do not explore the complementary strengths of low-cost SPAD and RGB sensors for diverse scene conditions in surface reconstruction. While some works have explored using RGB and SPAD sensors together, they primarily focus on improving depth estimation \cite{li2022deltar, meuleman2022floatingfusion}. Instead, in this work, we focus on leveraging the complementary strengths of RGB and low-cost SPADs to handle a complex mix of high and low-texture features within scenes.

Neural Radiance Fields (NeRF) have emerged as a foundational approach for learning volumetric scene representations from 2D images, enabling photorealistic view synthesis \cite{mildenhall2021nerf}. Subsequent work has focused on integrating surface geometry by learning implicit surfaces, enhancing reconstruction quality with normal predictions and volume rendering techniques \cite{wang2021neus}. More efficient representations, such as 3D Gaussian Splatting \cite{kerbl20233d}, have emerged for real-time rendering, with recent works extending 3DGS by estimating high-fidelity 3D surfaces using 2D ``Surfels" \cite{dai2024high}. 

Sensor fusion methods harnessing NeRF have shown promise in autonomous vehicle (AV) and robotics applications by combining radiance fields with depth data from time-of-flight sensors \cite{malik2024transient}. However, these works primarily focus on high-end, scanning laser experimental setups and overlook the potential of low-cost, small-form-factor single-photon sensors, which could be more accessible for mobile and robotic applications. Alternatively, several techniques for depth-supervised NeRFs have been proposed \cite{deng2022depth,song2023darf}, yet these methods rely on RGB-based cues from COLMAP \cite{schonberger2016structure} or monocular depth estimation, which are limited by the common pitfalls of RGB sensing on textureless surfaces or low-light settings. 

==> sec/old/4_method_old.tex <==
\section{Mixed-Texture Surface Reconstruction with Low-Cost SPADs and RGB}
\label{sec:method}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=1.0\textwidth]{figures/method.png} 
   \caption{Methods figure. \sid{The explanation of the transient and RGB input data is a bit confusing. For the transient, you could show a 3D space-time volumetric cube, then show the x-t and x-y slice/projection. The way it's combined with RGB right now is also not entirely clear right now. Don't think you need the SPAD and RGB image right (don't think it adds much to explaining the concept.} \sid{Word choice could also be more precise. You're not sampling a transient: you're sampling rays within a cone, then rendering a transient from those rays by summing up their individual transient responses.} \sid{Good to explicitly label outputs (depth, normals, RGB).}}
  \label{fig:methods}
\end{figure*}


\subsection{Surfel-Based Transient Rendering}

We follow the representation of Gaussian surfels introduced by \cite{dai2024high}. Surfels are represented by unstructured Gaussian kernels, each described by a set of parameters $\{ \mathbf{x}_i, r_i, \mathbf{s}_i, o_i, C_i \}$, for each Gaussian $i$ with kernel position $\mathbf{x}_i \in \mathbb{R}^3$, quaternion rotation $\mathbf{r}_i \in \mathbb{R}^4$, scaling factors  $\mathbf{s}_i \in \mathbb{R}^3$, opacity $o_i \in \mathbb{R}$, and spherical harmonic coefficients $C_i \in \mathbb{R}^k$. Using covariance matrix $\Sigma_i$ as the product of scaling matrix $\mathbf{S}_i$ and rotation matrix $\mathbf{R}(\mathbf{r}_i)$, we set $\mathbf{s}_i = [\mathbf{s}_i^x, \mathbf{s}_i^y, 0]^\top$ to get the 3D Gaussian surfel distribution represented as: 

\vspace{-2mm}
\begin{equation}
G(\mathbf{x}; \mathbf{x}_i, \Sigma_i) = \exp \left\{ -0.5 (\mathbf{x} - \mathbf{x}_i)^\top \Sigma_i^{-1} (\mathbf{x} - \mathbf{x}_i) \right\}    
\end{equation}
\vspace{-4mm}
\begin{equation}
\begin{aligned}
    \text{for} \quad \Sigma_i &= R(r_i) \mathbf{S}_i \mathbf{S}_i^\top R(r_i)^\top, \\
     &= R(r_i) \text{Diag}\left[ (s_i^x)^2, (s_i^y)^2, 0 \right] R(r_i)^\top
\end{aligned}  
\end{equation}

Differentiable view rendering follows that of 3DGS, such that the color of each pixel $\mathbf{u}$ is computed:

\begin{equation}
\tilde{C} = \sum_{i=0}^{n} T_i \alpha_i c_i, \ \ T_i = \prod_{j=0}^{i-1} (1 - \alpha_j), \ \ \alpha_i = G'(\mathbf{u}; \mathbf{u}_i, \Sigma'_i) o_i
\end{equation}

where $\alpha_i$ is the alpha-blending weight and $c_i$ is the color computed from the spherical harmonics. The 3D Gaussian is reparameterized in 2D ray space as $G'$, with $\Sigma'$ the transformed covariance matrix in image coordinates: 

\begin{equation}
G'(\mathbf{u}; \mathbf{u}_i, \Sigma'_i) = \exp \left\{ -0.5 (\mathbf{u} - \mathbf{u}_i)^\top \Sigma_i'^{-1} (\mathbf{u} - \mathbf{u}_i) \right\}
\end{equation}

\begin{equation}
\Sigma'_i = \left( \mathbf{J}_k \mathbf{W}_k \Sigma_i \mathbf{W}_k^\top \mathbf{J}_k^\top \right) [: 2, : 2]
\end{equation}

Per-pixel normal $\tilde{N}$ and depth $\tilde{D}$ are then computed as:

{ 
\begin{equation}
\begin{aligned}
\tilde{N} = \frac{1}{1 - T_{n+1}} \sum_{i=0}^{n} T_i \alpha_i R_i[:, 2], 
\tilde{D} = \frac{1}{1 - T_{n+1}} \sum_{i=0}^{n} T_i \alpha_i d_i(\mathbf{u})
\end{aligned}  
\end{equation}
}

Dai et al. \cite{dai2024high} further introduce an updated depth rendering to calculate the intersection of each ray cast through pixel $\mathbf{u}$ with a (perhaps slanted) Gaussian ellipse as: 
$$
d_i(\mathbf{u}) = d_i(\mathbf{u}_i) + (W_k R_i)[2, :] J_{\text{pr}}^{-1} (\mathbf{u} - \mathbf{u}_i)
$$
where $J_{\text{pr}}^{-1}$ is the Jacobian of inverse mapping, and $(W_k R_i)$ transforms the rotation matrix to the camera space.

\sectionbf{Transient rendering with surfels} We then wish to synthesize transient images from a low-cost SPAD using the Gaussian surfel representations. For each pixel $\mathbf{u}$, the depth and opacity of each contributing surfel is stored in a buffer where $d_i(\mathbf{u})$ and $o_i$ represent the depth and opacity of surfel $i$ contributing to pixel $\mathbf{u}$. We then estimate the per-pixel transient using a differentiable soft-binning procedure. 

First, the depth range $[t_{\text{min}}, t_{\text{max}}]$ is divided into $n_{\text{bins}}$ with bin width $\Delta t$, matching the SPAD's timing resolution. For each surfel $i$ contributing to pixel $\mathbf{u}$, its depth $d_i(\mathbf{u})$ is assigned to a bin. The per-surfel $i$, per pixel $\mathbf{u}$ bin index $\beta_i(\mathbf{u})$ is computed as:

\begin{equation}
\beta_i(\mathbf{u}) = \left\lfloor \frac{d_i(\mathbf{u}) - t_{\text{min}}}{\Delta t} \right\rfloor
\end{equation}

We then apply an opacity-weighted soft histogramming to distribute surfel contribution across two adjacent bins; we find qualitativley that this improves gradient flow in rendering.  For lower bin $\beta_i(\mathbf{u})$ and upper bin $\beta_i(\mathbf{u}) + 1$ \sid{what is lower bin and upper bin?}, we compute the per-surfel opacity-weighted contributions as: 

\begin{equation}
w_{i,\text{low}} = 1 - \left( \frac{d_i(\mathbf{u}) - t_{\text{min}}}{\Delta t} - \beta_i(\mathbf{u}) \right), w_{i,\text{up}} = 1 - w_{i,\text{low}}
\end{equation}

\sid{what is $w_i$?} The final depth histogram $H_{\mathbf{d}}[b](\mathbf{u})$, for each bin $b$ at pixel $\mathbf{u}$, is constructed by summing the opacity-weighted contributions across all surfels:

\begin{equation}
\begin{aligned}
H_{\mathbf{d}}[b](\mathbf{u}) = & \sum_{i} \left( w_{i,\text{low}} \cdot o_i \, \delta[b = \beta_i(\mathbf{u})] \right. \\
& \left. + w_{i,\text{up}} \cdot o_i \, \delta[b = \beta_i(\mathbf{u}) + 1] \right)
\end{aligned}
\end{equation}



\subsection{RGB and Transient Loss Signal}

\sectionbf{Optimization} (r1 rgb, kl divergence, ...) 


We define two primary loss functions: one for RGB color fidelity and another for transient histogram accuracy. These losses guide the optimization of both the standard image reconstruction and the transient rendering process.

\textbf{RGB Loss}

For the RGB rendering, we use a combination of L1 loss and the Structural Similarity Index (SSIM), providing a balance between pixel-wise accuracy and perceptual quality. The L1 loss between the rendered image $\mathbf{C}$ and the ground truth $\mathbf{C}_{gt}$ is weighted by an upscaled color variance mask $\mathbf{w}_{\text{color}}$ to account for varying importance across image regions. The total RGB loss is:

\begin{equation}
\mathcal{L}_{\text{RGB}} = (1 - \lambda_{\text{SSIM}}) \| \mathbf{C} - \mathbf{C}_{gt} \|_1 + \lambda_{\text{SSIM}} (1 - \text{SSIM}(\mathbf{C}, \mathbf{C}_{gt}))
\end{equation}

where $\lambda_{\text{SSIM}}$ controls the trade-off between the L1 and SSIM losses.

\textbf{Transient Loss}

For transient rendering, we compute the Kullback-Leibler (KL) divergence between the predicted normalized depth histogram $\mathbf{H}_{d}^\text{log}$ and the ground truth transient histogram $\mathbf{H}_{\text{gt}}$. The transient loss is:

\begin{equation}
\mathcal{L}_{\text{transient}} = \frac{1}{N} \sum_i \text{KL}(\mathbf{H}_{d,i}^{\text{log}} \parallel \mathbf{H}_{\text{gt},i})
\end{equation}

where $N$ is the number of pixels.

\sectionbf{Texture Variance-Based Weighting}

\sectionbf{Pruning and Densifying}


